The Origin of the Intrinsic Scatter in the Relation Between Black Hole Mass and Bulge Luminosity for Nearby Active Galaxies

We investigate the origin of the intrinsic scatter in the correlation between black hole mass (MBH) and bulge luminosity [L(bulge)] in a sample of 45 massive, local (z < 0.35) type~1 active galactic nuclei (AGNs). We derive MBH from published optical spectra assuming a spherical broad-line region, and L(bulge) from detailed two-dimensional decomposition of archival optical Hubble Space Telescope images. AGNs follow the MBH-L(bulge) relation of inactive galaxies, but the zero point is shifted by an average of \Delta log MBH ~ -0.3 dex. We show that the magnitude of the zero point offset, which is responsible for the intrinsic scatter in the MBH-L(bulge) relation, is correlated with several AGN and host galaxy properties, all of which are ultimately related to, or directly impact, the BH mass accretion rate. At a given bulge luminosity, sources with higher Eddington ratios have lower MBH. The zero point offset can be explained by a change in the normalization of the virial product used to estimate MBH, in conjunction with modest BH growth (~ 10%--40%) during the AGN phase. Galaxy mergers and tidal interactions appear to play an important role in regulating AGN fueling in low-redshift AGNs.

==> tab1.tex <==
%\documentclass[12pt,preprint]{aastex}
%\begin{document}
\def\nd{\nodata}
\pagestyle{empty}
\begin{deluxetable}{lccccccccccccc}
\tablecolumns{14}
\tabletypesize{\scriptsize}
\rotate
\tablewidth{8.5in}
\tablecaption{The sample}
\tablehead{
\colhead{ Source Name} &
\colhead{ $z$} &
\colhead{ $D_{L}$} &
\colhead{ Line} &
\colhead{ FWHM} &
\colhead{ Ref.} &
\colhead{ log $\lambda L_{5100}^{\rm spec}$} &
\colhead{ Ref.} &
\colhead{ log $\lambda L_{5100}^{\rm image}$} &
\colhead{ log $M_{\rm BH}$} &
\colhead{ Method} &
\colhead{ $L_{\rm bol}/L_{\rm Edd}$} &
\colhead{ log $P^{\rm tot}_{6 {\rm cm}}$} &
\colhead{ Ref.} \\
\colhead{ } &
\colhead{ } &
\colhead{ (Mpc)} &
\colhead{ } &
\colhead{ (km s$^{-1}$)} &
\colhead{ } &
\colhead{ (ergs s$^{-1}$)} &
\colhead{ } &
\colhead{ (ergs s$^{-1}$)} &
\colhead{ $(M_{\odot})$} &
\colhead{ } &
\colhead{ } &
\colhead{ (W Hz$^{-1}$)} &
\colhead{ } \\
\colhead{ (1)} &
\colhead{ (2)} &
\colhead{ (3)} &
\colhead{ (4)} &
\colhead{ (5)} &
\colhead{ (6)} &
\colhead{ (7)} &
\colhead{ (8)} &
\colhead{ (9)} &
\colhead{ (10)} &
\colhead{ (11)} &
\colhead{ (12)} &
\colhead{ (13)} &
\colhead{  (14) }
}
\startdata
3C 59&0.109& 499.4&H$\alpha$&9800&1&43.94&1&44.13&$ 8.85_{- 0.20}^{+ 0.20}$ &S&0.01&25.27&1\nl
E1821+643&0.297&1526.8&H$\beta$&5190&2&\nd&\nd&45.75&$ 9.08_{- 0.20}^{+ 0.20}$ &S&0.34&\nd&\nd\nl
Fairall 9&0.047& 205.9&H$\beta$&5900&3&44.25&2&42.98&$ 8.15_{- 0.09}^{+ 0.09}$ &R&0.09&\nd&\nd\nl
$[$HB89$]$ 0316$-$346&0.265&1338.5&H$\beta$&7048&4&\nd&\nd&44.72&$ 8.81_{- 0.30}^{+ 0.30}$ &S&0.06&\nd&\nd\nl
$[$HB89$]$ 2201+315&0.295&1514.9&H$\beta$&3320&4&\nd&\nd&45.24&$ 8.43_{- 0.30}^{+ 0.30}$ &S&0.47&26.93&2\nl
HE 0306$-$3301&0.247&1234.8&H$\beta$&2346&5&\nd&\nd&44.79&$ 7.89_{- 0.20}^{+ 0.20}$ &S&0.57&\nd&\nd\nl
HE 0354$-$5500&0.267&1350.1&H$\beta$&2264&5&\nd&\nd&44.72&$ 7.83_{- 0.20}^{+ 0.20}$ &S&0.56&23.92&3\nl
HE 1434$-$1600&0.142& 665.3&H$\beta$&7068&5&\nd&\nd&44.38&$ 8.64_{- 0.20}^{+ 0.20}$ &S&0.04&23.30&4\nl
MC 1635+119&0.146& 685.8&H$\beta$&5271&4&44.06&1&43.50&$ 7.92_{- 0.20}^{+ 0.20}$ &S&0.05&24.43&2\nl
MRK 1048 &0.043& 188.2&H$\beta$&7498&4&43.85&3&43.73&$ 8.35_{- 0.20}^{+ 0.20}$ &S&0.02&21.92&5\nl
MS 0244.8+1928&0.176& 842.9&H$\beta$&3700&6&44.37&1&44.36&$ 8.06_{- 0.20}^{+ 0.20}$ &S&0.14&\nd&\nd\nl
MS 0754.6+3928&0.096& 435.8&H$\beta$&2123&4&\nd&\nd&44.71&$ 7.76_{- 0.20}^{+ 0.20}$ &S&0.73&23.45&6\nl
MS 1059.0+7302&0.089& 402.0&H$\beta$&7690&4&\nd&\nd&43.48&$ 8.24_{- 0.20}^{+ 0.20}$ &S&0.01&\nd&\nd\nl
MS 1545.3+0305&0.098& 445.5&H$\beta$&5868&7&\nd&\nd&43.22&$ 7.87_{- 0.20}^{+ 0.20}$ &S&0.02&\nd&\nd\nl
OX 169 &0.211&1032.6&H$\beta$&5030&4&45.18&1&44.72&$ 8.52_{- 0.20}^{+ 0.20}$ &S&0.19&26.11&2\nl
PG 0052+251&0.155& 732.4&H$\beta$&4165&3&44.96&2&44.64&$ 8.31_{- 0.10}^{+ 0.10}$ &R&0.32&22.65&7\nl
PG 0804+761&0.100& 455.3&H$\beta$&2012&3&44.94&2&44.96&$ 8.58_{- 0.05}^{+ 0.05}$ &R&0.16&22.75&7\nl
PG 0923+201&0.190& 918.0&H$\beta$&7233&4&44.88&1&44.74&$ 8.84_{- 0.20}^{+ 0.20}$ &S&0.07&22.38&7\nl
PG 0953+414&0.234&1161.0&H$\beta$&3140&3&45.22&2&45.09&$ 8.18_{- 0.08}^{+ 0.08}$ &R&0.77&23.46&7\nl
PG 1004+130&0.240&1195.0&H$\beta$&6215&4&45.29&1&45.18&$ 8.94_{- 0.20}^{+ 0.20}$ &S&0.14&22.85&7\nl
PG 1012+008&0.186& 896.4&H$\beta$&2604&4&44.47&1&44.44&$ 7.80_{- 0.20}^{+ 0.20}$ &S&0.32&22.96&7\nl
PG 1116+215&0.176& 842.9&H$\beta$&3054&4&45.40&4&45.00&$ 8.23_{- 0.20}^{+ 0.20}$ &S&0.65&23.38&7\nl
PG 1202+281&0.165& 784.7&H$\beta$&4931&4&44.60&4&44.49&$ 8.38_{- 0.30}^{+ 0.30}$ &S&0.10&22.79&7\nl
PG 1211+143&0.080& 359.1&H$\beta$&1317&3&44.75&2&44.58&$ 7.90_{- 0.11}^{+ 0.11}$ &R&0.50&24.36&7\nl
PG 1226+023 &0.158& 748.0&H$\beta$&2598&3&45.96&2&45.79&$ 8.69_{- 0.08}^{+ 0.08}$ &R&1.32&27.37&7\nl
PG 1302$-$102&0.278&1414.4&H$\beta$&3758&4&45.83&4&45.34&$ 8.58_{- 0.30}^{+ 0.30}$ &S&0.40&26.27&7\nl
PG 1307+085&0.155& 732.4&H$\beta$&5058&3&44.88&2&44.64&$ 8.38_{- 0.11}^{+ 0.11}$ &R&0.22&22.32&7\nl
PG 1309+355&0.184& 885.7&H$\beta$&3974&4&45.01&4&44.85&$ 8.38_{- 0.30}^{+ 0.30}$ &S&0.25&24.70&7\nl
PG 1351+640&0.088& 397.2&H$\beta$&5579&4&44.05&4&44.47&$ 8.48_{- 0.20}^{+ 0.20}$ &S&0.04&21.99&7\nl
PG 1411+442&0.089& 402.0&H$\beta$&2398&3&44.63&2&44.50&$ 8.39_{- 0.12}^{+ 0.12}$ &R&0.12&22.07&7\nl
PG 1416$-$129 &0.129& 599.1&H$\beta$&6283&4&45.14&4&44.14&$ 8.41_{- 0.30}^{+ 0.30}$ &S&0.12&23.19&7\nl
PG 1426+015 &0.086& 387.7&H$\beta$&6323&3&44.72&2&44.46&$ 8.85_{- 0.12}^{+ 0.12}$ &R&0.05&22.31&7\nl
PG 1444+407&0.267&1350.1&H$\beta$&2944&4&45.20&4&45.00&$ 8.21_{- 0.20}^{+ 0.20}$ &S&0.56&22.54&7\nl
PG 1613+658&0.129& 599.1&H$\beta$&7897&3&44.98&2&44.80&$ 8.19_{- 0.10}^{+ 0.10}$ &R&0.44&23.11&7\nl
PG 1617+175 &0.112& 514.2&H$\beta$&4718&3&44.48&2&44.37&$ 8.51_{- 0.09}^{+ 0.09}$ &R&0.07&22.51&7\nl
PG 1700+518&0.292&1497.0&H$\beta$&1846&3&45.63&2&45.37&$ 8.63_{- 0.10}^{+ 0.09}$ &R&0.71&24.29&7\nl
PG 2130+099&0.062& 274.6&H$\beta$&2912&3&44.46&2&44.48&$ 8.40_{- 0.05}^{+ 0.05}$ &R&0.08&22.24&7\nl
PHL 909&0.171& 816.4&H$\beta$&9660&6&44.47&1&44.78&$ 9.12_{- 0.20}^{+ 0.20}$ &S&0.02&23.02&8\nl
PHL 1093 &0.260&1309.5&H$\beta$&7610&6&44.30&1&44.31&$ 8.66_{- 0.20}^{+ 0.20}$ &S&0.03&26.07&4\nl
PKS 0736+01&0.191& 923.4&H$\beta$&3259&4&44.58&1&44.61&$ 8.08_{- 0.20}^{+ 0.20}$ &S&0.23&26.22&2\nl
PKS 1020$-$103&0.197& 955.9&H$\beta$&7950&6&43.88&1&44.29&$ 8.69_{- 0.20}^{+ 0.20}$ &S&0.02&25.68&9\nl
PKS 1217+02&0.239&1189.3&H$\beta$&3830&6&44.89&1&44.66&$ 8.25_{- 0.20}^{+ 0.20}$ &S&0.24&25.87&8\nl
PKS 2135$-$14&0.200& 972.3&H$\beta$&9294&4&45.18&1&44.54&$ 8.96_{- 0.20}^{+ 0.20}$ &S&0.06&26.16&9\nl
PKS 2349$-$01&0.174& 832.3&H$\beta$&5511&4&44.97&1&44.63&$ 8.55_{- 0.20}^{+ 0.20}$ &S&0.12&25.73&10\nl
PKS 2355$-$082&0.211&1032.6&H$\beta$&7510&6&43.98&1&44.12&$ 8.56_{- 0.20}^{+ 0.20}$ &S&0.02&25.30&10\nl
\enddata
\tablecomments{
Col. (1): Object name.
Col. (2): Redshift.
Col. (3): Luminosity distance.
Col. (4): Broad emission line used to estimate black hole mass.
Col. (5): Full width at half maximum of broad emission line.
Col. (6): Reference for FWHM:
(1) Eracleous \& Halpern 1994;
(2) Zheng et al. 2002;
(3) Peterson et al. 2004;
(4) Marziani et al. 2003;
(5) Letawe et al. 2008;
(6) McLure \& Dunlop 2001;
(7) Boroson 2005.
Col. (7): Continuum luminosity at 5100 \AA\ derived from observed spectrum.
Col. (8): Reference for $\lambda L_{5100}^{\rm spec}$:
(1) McLure \& Dunlop 2001;
(2) Peterson et al. 2004;
(3) Grupe et al. 2004;
%(4) Marziani et al. 2003;
(4) Vestergaard \& Peterson 2006.
Col. (9): Continuum luminosity at 5100 \AA\ derived from the best-fit
GALFIT model.
Col. (10): Black hole mass.
%XX switch col. 11 and col. 12
Col. (11): Method for estimating $M_{\rm BH}$:
S = virial method based on the single-epoch spectrum; 
R = reverberation mapping method.
Col. (12): Eddington ratio, where $L_{\rm bol} = 9 \lambda
L_{\lambda}$(5100 \AA).
Col. (13): Radio power at 6 cm; for observations done at other wavelengths,
we extrapolate to 6 cm assuming $f_\nu \propto \nu^{-0.5}$.
Col. (14): Reference for $P^{\rm tot}_{6 {\rm cm}}$:
(1) Kellermann \& Pauliny-Toth 1973;
(2) Becker et al. 1991;
(3) Mauch et al. 2003;
(4) Condon et al. 1998;
%(4) NVSS;
%XX isn't NVSS the same as Condon et al. 1998?
(5) Barvainis \& Antonucci 1989;
(6) Becker et al. 1995;
(7) Kellermann et al. 1989.;
(8) Bennett et al. 1986;
(9) Griffith et al. 1994;
%(11) K\"{u}hr et al. 1981;
(10) Griffith et al. 1995.
}
\end{deluxetable}
%\end{document}


==> tab2.tex <==
%\documentclass[12pt,preprint]{aastex}
%\begin{document}
\def\ser{S\'{e}rsic}
\def\asec{$^{\prime\prime}$}
\def\h{\hskip -1.5 mm}
\def\ha{\hskip -3 mm}
\def\hb{\hskip -8 mm}
\def\nd{\nodata}
\pagestyle{empty}
\begin{deluxetable}{lcrccccccccccccccccc}
%\ptlandscape
%\textheight=8.2in
%\voffset=-1.5in
\tablecolumns{20}
\tablenum{2}
\tabletypesize{\scriptsize}
\rotate
\tablewidth{0pc}
\tablecaption{Fitted Parameters}
\tablehead{
\colhead{}  &  
\colhead{\h}  &
\colhead{\h}  &
\colhead{\h}  &
\multicolumn{4}{c}{\h Bulge} & 
\colhead{\h}   &
\multicolumn{4}{c}{\h Disk or Tidal Feature\tablenotemark{a}} &
\colhead{\h}   &
\multicolumn{3}{c}{\h Host} &
\colhead{\h}   &
\colhead{\h}   &
\colhead{\h}   \\
\cline{5-8} \cline{10-13} \cline{15-17} \\
\colhead{ Name} &
\colhead{ \h Detector/Filter} &
\colhead{ \h Exp.} &
\colhead{ \h $m_{\rm nuc}$} &
\colhead{ \h $m_{\rm bul}$} &
\colhead{ \h $R_e$} &
\colhead{ \h $n$} &
\colhead{ \h $\mu_e$} &
\colhead{ \h} &
\colhead{ \h $m_{\rm disk}$} &
\colhead{ \h $R_e$} &
\colhead{ \h $n$} &
\colhead{ \h $\mu_e$} &
\colhead{ \h} &
\colhead{ \h $m_{\rm host}$} &
\colhead{ \h $m_{\rm aper}$} &
\colhead{ \h $B/T$} &
\colhead{ \h} &
\colhead{ \h $a_1$} &
\colhead{ \h Qual.} \\
\colhead{ } &
\colhead{ \h} &
\colhead{ \h (s) } &
\colhead{ \h (mag) } &
\colhead{ \h (mag) } &
\colhead{ \h (\asec) } &
\colhead{ \h } &
\colhead{ \h } &
\colhead{ \h } &
\colhead{ \h (mag)} &
\colhead{ \h (\asec) } &
\colhead{ \h } &
\colhead{ \h } &
\colhead{ \h } &
\colhead{ \h (mag)} &
\colhead{ \h (mag)} &
\colhead{ \h} &
\colhead{ \h} &
\colhead{ \h}   \\
\colhead{ (1)} &
\colhead{ \h (2)} &
\colhead{ \h (3) } &
\colhead{ \h (4) } &
\colhead{ \h (5) } &
\colhead{ \h (6)} &
\colhead{ \h (7)} &
\colhead{ \h (8)} &
\colhead{ \h } &
\colhead{ \h (9)} &
\colhead{ \h (10)} &
\colhead{ \h (11)} &
\colhead{ \h (12)} &
\colhead{ \h } &
\colhead{ \h (13)} &
\colhead{ \h (14)} &
\colhead{ \h (15)} &
\colhead{ \h} &
\colhead{ \h (16)} &
\colhead{ \h (17)}
}
\startdata
3C 59                &\h WF2/F675W &\h 1800&\h 15.94&\h 15.87&\h 3.41&\h 4.00 
&\h 21.93&\h&\h$\leq20.5$ &\h\nd   &\h \nd &\h \nd  &\h&\h 15.87&\h 15.9
&\h 1($\geq0.99$)    &\h&\h 0.01   &\h N  \nl
E1821+643            &\h WF3/F791W &\h 3900&\h 13.51&\h 15.97&\h 4.31&\h 4.00 
&\h 22.53&\h&\h$\leq19.0$ &\h\nd   &\h \nd &\h \nd  &\h&\h 15.97&\h 15.6–-16.3
&\h 1($\geq0.94$) &\h&\h 0.17      &\h N \nl
Fairall 9            &\h HRC/F550M &\h 1020&\h 17.97&\h 15.83&\h 0.04&\h 4.00 
&\h 12.18&\h&\h 16.45&\h 1.78      &\h1.00 &\h 20.40&\h&\h 15.35&\h 15.2–-15.5 
&\h 0.64          &\h&\h0.03       &\h N \nl
$[$HB89$]$ 0316$−-$346&\h WF3/F606W &\h 1400&\h 16.53&\h 18.57&\h 1.34&\h 3.00
&\h 22.44&\h&\h 19.92&\h 1.28      &\h 0.73&\h 23.01&\h&\h 18.06&\h\nd 
&\h 0.63          &\h&\h 0.18      &\h S \\
$[$HB89$]$ 2201+315  &\h PC/F702W  &\h 560 &\h 15.41&\h 17.34&\h 0.78&\h 4.00
&\h 20.18&\h&\h$\leq20.0$ &\h \nd  &\h\nd  &\h \nd  &\h&\h 17.34&\h\nd 
&\h 1($\geq0.92$) &\h&\h 0.09      &\h S \\
$[$HB89$]$ 2201+315  &\h PC/F555W  &\h 2700&\h 15.95&\h 17.87&\h 1.38&\h 4.00
&\h 21.96&\h&\h$\leq20.0$ &\h\nd   &\h\nd  &\h\nd   &\h&\h 17.87&\h\nd
&\h 1($\geq0.88$) &\h&\h0.01       &\h S \\
HE 0306$−-$3301      &\h HRC/F606W &\h 990 &\h 16.29&\h 19.49&\h 0.68&\h 4.00 
&\h 22.04&\h&\h 18.47&\h 1.33      &\h1.00 &\h21.79 &\h&\h 18.11&\h 17.5–-18.2 
&\h 0.28          &\h&\h0.06       &\h N \\
HE 0354$−-$5500   &\h HRC/F606W &\h 1200&\h 16.56&\h 18.19&\h 0.58&\h 4.00
&\h 22.40&\h&\h 20.98&\h \nd       &\h \nd &\h \nd  &\h&\h 18.11&\h 17.4–-18.2 
&\h 0.93          &\h&\h 0.33      &\h N \\
HE 1434$−-$1600      &\h HRC/F606W &\h 990 &\h 16.43&\h 17.54&\h 1.85&\h 4.00
&\h 22.27&\h&\h$\leq21.0$ &\h\nd   &\h\nd  &\h\nd   &\h&\h 17.54&\h 17.2–-17.4
&\h 1($\geq0.96$)    &\h&\h 0.01      &\h N \\
MC 1635+119          &\h WF2/F675W &\h 1800&\h 18.19&\h 16.80&\h 1.76&\h 4.00 
&\h 21.42&\h&\h$\leq21.0$ &\h\nd   &\h\nd  &\h\nd   &\h&\h 16.80&\h 16.7 
&\h 1($\geq0.98$) &\h&\h 0.01      &\h N \\
MRK 1048             &\h PC6/F785LP&\h 230 &\h 14.91&\h 13.69&\h 1.61&\h 4.00
&\h 18.12&\h&\h 14.52&\h 14.05     &\h 1.00&\h 22.95&\h&\h 13.28&\h 13.3
&\h 0.68          &\h&\h 1.86      &\h N \\
MS 0244.8+1928  &\h WF2/F675W &\h 1800&\h 16.82&\h 17.55&\h 2.07&\h 4.00
&\h 22.52&\h&\h$\leq20.5$ &\h\nd   &\h\nd  &\h\nd   &\h&\h 17.55&\h 17.5
&\h 1($\geq0.94$) &\h&\h 0.04      &\h N \\
MS 0754.6+3928       &\h PC/F814W  &\h 600 &\h 13.70&\h 15.94&\h 2.34&\h 4.00
&\h 21.18&\h&\h$\leq18.0$ &\h\nd   &\h\nd  &\h\nd   &\h&\h 15.94&\h 15.9
&\h 1($\geq0.87$) &\h&\h 0.09      &\h N \\
MS 1059.0+7302       &\h PC/F814W  &\h 600 &\h 16.61&\h 17.02&\h 0.38&\h 3.94
&\h 18.33&\h&\h 15.89&\h 2.76      &\h 1.00&\h 20.80&\h&\h 15.57&\h 15.6
&\h 0.26          &\h&\h 0.00      &\h N \\
MS 1545.3+0305       &\h PC/F814W  &\h 600 &\h 17.57&\h 16.30&\h 1.09&\h 4.00
&\h 19.89&\h&\h 16.20&\h 3.23      &\h 1.00&\h 21.44&\h&\h 15.50&\h 15.5
&\h 0.47          &\h&\h 0.36      &\h N \\
OX 169               &\h WF2/F675W &\h 1800&\h 16.02&\h 17.33&\h 1.05&\h 4.00
&\h 20.82&\h&\h 19.05&\h \nd       &\h \nd &\h \nd  &\h&\h 17.13&\h 16.8–-16.9
&\h 0.83          &\h&\h 0.29      &\h N \\
PG 0052+251          &\h WF2/F675W &\h 1800&\h 15.48&\h 16.95&\h 1.38&\h 4.00
&\h 21.02&\h&\h 17.72&\h 3.99      &\h 0.20&\h 22.86&\h&\h 16.51&\h 16.3–-16.4 
&\h 0.67          &\h&\h 0.22      &\h N \\
%PG 0157+001          &\h WF2/F675W &\h 1800&\h 16.03&\h 17.02&\h 0.75&\h 1.00
%&\h 19.10&\h&\h 15.92&\h 6.95      &\h 1.23&\h 22.93&\h&\h 15.58&\h 15.4–-15.5 
%&\h 0.27          &\h&\h 0.15      &\h N \\
PG 0804+761      &\h WFC/F625W &\h 1590&\h 13.95&\h 16.83&\h 1.75&\h 4.00
&\h 21.44&\h&\h 19.06&\h 2.17      &\h 0.22&\h 22.88&\h&\h 16.70&\h 16.4 
&\h 0.89          &\h&\h 0.01      &\h N \\
PG 0923+201          &\h WF2/F675W &\h 1800&\h 15.66&\h 17.22&\h 2.04&\h 4.00
&\h 22.16&\h&\h$\leq20.0$ &\h\nd   &\h\nd  &\h\nd   &\h&\h 17.22&\h 16.8–-17.2 
&\h 1($\geq0.93$) &\h&\h 0.00      &\h N \\
PG 0953+414          &\h WF2/F675W &\h 1800&\h 15.11&\h 18.03&\h 2.61&\h 4.00
&\h 23.50&\h&\h$\leq21.5$ &\h\nd   &\h\nd  &\h\nd   &\h&\h 18.03&\h 17.9–-18.7 
&\h 1($\geq0.96$) &\h&\h 0.12      &\h N \\
PG 1004+130          &\h WF2/F675W &\h 1800&\h 15.04&\h 16.79&\h 2.05&\h 4.00
&\h 21.73&\h&\h$\leq21.5$ &\h\nd   &\h\nd  &\h\nd   &\h&\h 16.79&\h 16.7–-16.9 
&\h1($\geq0.99$)  &\h&\h 0.04      &\h N \\
PG 1012+008          &\h WF2/F675W &\h 1800&\h 16.33&\h 17.08&\h 2.96&\h 3.24
&\h 22.72&\h&\h\nd   &\h\nd        &\h\nd  &\h\nd   &\h&\h 17.08&\h 15.9–-16.0 
&\h 1             &\h&\h 0.31      &\h N \\
PG 1116+215          &\h WF3/F606W &\h 2200&\h 15.27&\h 17.01&\h 1.99&\h 4.00
&\h 21.90&\h&\h$\leq20.5$ &\h\nd   &\h\nd  &\h\nd   &\h&\h 17.01&\h 16.6–-16.9
&\h 1($\geq0.96$) &\h&\h 0.02    &\h N \\
PG 1202+281          &\h WF3/F606W &\h1800 &\h 16.25&\h 17.63&\h 1.33&\h 4.00
&\h 21.64&\h&\h$\leq20.5$ &\h\nd   &\h\nd  &\h\nd   &\h&\h 17.63&\h\nd 
&\h 1($\geq0.93$) &\h&\h 0.00      &\h N \\
PG 1211+143          &\h WFC/F625W &\h 1590&\h 14.33&\h 16.94&\h 0.95&\h 5.84
&\h 20.42&\h&\h 18.21&\h 4.72      &\h 0.32&\h 23.81&\h&\h 16.57&\h 15.7–-16.0 
&\h 0.72          &\h&\h 0.03      &\h N \\
                     &\h           &\h     &\h      &\h      &\h     &\h       
&\h      &\h&\h 19.60&\h 1.40      &\h 0.15&\h 23.43&\h&\h      &\h            
&\h               &\h&\h           &\h  \\
PG 1226+023          &\h WF3/F606W &\h 2200&\h 12.86&\h 16.06&\h 6.28&\h 4.00 
&\h 23.44&\h&\h\nd   &\h\nd        &\h\nd  &\h\nd   &\h&\h 16.06&\h\nd 
&\h 1             &\h&\h 0.13      &\h P \\
PG 1302$-−$102        &\h WF3/F606W &\h 1800&\h 15.12&\h 17.73&\h 1.03&\h 4.00
&\h 21.19&\h&\h$\leq21.0$ &\h\nd   &\h\nd  &\h\nd   &\h&\h 17.73&\h\nd 
&\h 1($\geq0.95$) &\h&\h 0.00      &\h S \\
PG 1302$−-$102        &\h PC/F702W  &\h 1800&\h 14.94&\h 17.34&\h 2.03&\h 4.00
&\h 22.27&\h&\h$\leq20.5$ &\h\nd   &\h\nd  &\h\nd   &\h&\h 17.34&\h\nd 
&\h 1($\geq0.95$) &\h&\h 0.01      &\h S \\
PG 1307+085          &\h WF3/F606W &\h 1400&\h 15.72&\h 17.72&\h 0.94&\h 4.00
&\h 20.96&\h&\h$\leq21.5$ &\h\nd   &\h\nd  &\h\nd   &\h&\h 17.72&\h 17.7
&\h 1($\geq0.97$) &\h&\h 0.07      &\h S \\
PG 1309+355          &\h WF3/F606W &\h 2100&\h 15.50&\h 16.74&\h 1.58&\h 4.00
&\h 21.12&\h&\h$\leq21.0$ &\h\nd   &\h\nd  &\h\nd   &\h&\h 16.74&\h\nd 
&\h 1($\geq0.98$) &\h&\h 0.01      &\h S \\
PG 1351+640          &\h WFC/F625W &\h 1800&\h 14.85&\h 16.07&\h 1.96&\h 3.81
&\h 20.90&\h&\h 18.75&\h 1.41      &\h 1.00&\h 22.19&\h&\h 15.98&\h 15.5
&\h 0.92          &\h&\h 0.09      &\h N \\
PG 1411+442          &\h WFC/F625W &\h 1680&\h 14.76&\h 16.96&\h 1.12&\h 4.00
&\h 20.60&\h&\h 16.68&\h 8.08      &\h 1.38&\h 24.06&\h&\h 16.06&\h 15.8--16.4
&\h 0.43          &\h&\h 0.21      &\h N \\
PG 1416$-$129        &\h PC/F814W  &\h 600 &\h 15.84&\h 17.01&\h 3.09&\h 4.00
&\h 22.84&\h&\h$\leq20.0$ &\h\nd   &\h\nd  &\h\nd   &\h&\h 17.01&\h 16.1–-16.8
&\h 1($\geq0.94$) &\h&\h 0.00      &\h S \\
PG 1426+015          &\h PC/F814W  &\h 600 &\h 14.02&\h 16.08&\h 0.61&\h 2.12
&\h 18.08&\h&\h 15.26&\h 4.11      &\h 0.71&\h 20.87&\h&\h 14.84&\h 14.3–-14.7
&\h 0.32          &\h&\h 0.12      &\h N \\
PG 1444+407          &\h WF3/F606W &\h 2300&\h 15.81&\h 18.68&\h 0.85&\h 4.00
&\h 21.71&\h&\h 19.08&\h 2.47      &\h 0.31&\h 23.26&\h&\h 18.10&\h 17.5–-17.8
&\h 0.59          &\h&\h 0.10      &\h N \\
PG 1613+658          &\h WFC/F625W &\h 1860&\h 14.87&\h 15.92&\h 3.00&\h 4.00
&\h 21.69&\h&\h 16.25&\h 4.89      &\h 1.00&\h 22.39&\h&\h 15.31&\h 15.0–-15.1
&\h 0.58          &\h&\h 0.40      &\h N \\
PG 1617+175          &\h WFC/F625W &\h 1590&\h 15.69&\h 17.70&\h 1.37&\h 4.00
&\h 21.78&\h&\h 19.51&\h 1.83      &\h 0.22&\h 22.98&\h&\h 17.51&\h 17.4–-17.5
&\h 0.84          &\h&\h 0.10      &\h N \\
PG 1700+518          &\h PC/F547M  &\h 2000&\h 15.45&\h 17.78&\h 1.15&\h 4.00
&\h 21.47&\h&\h 19.82&\h \nd       &\h \nd &\h \nd  &\h&\h 17.63&\h 16.0–-17.3
&\h 0.87             &\h&\h 0.39      &\h N \\
PG 2130+099          &\h WF2/F555W &\h 1800&\h 14.47&\h 17.34&\h 2.31&\h 0.44
&\h 21.51&\h&\h 16.49&\h 12.85     &\h 0.33&\h 24.28&\h&\h 16.08&\h 16.0
&\h 0.31          &\h&\h0.23       &\h S \\
PHL 909              &\h WF2/F675W &\h 1800&\h 15.51&\h 16.60&\h 2.72&\h 4.00
&\h 22.16&\h&\h$\leq21.5$ &\h\nd   &\h\nd  &\h\nd   &\h&\h 16.60&\h 16.1–-16.6
&\h 1($\geq0.99$)    &\h&\h0.10    &\h N \\
PHL 1093             &\h WF2/F675W &\h 1800&\h 17.27&\h 17.23&\h 2.24&\h 4.00
&\h 22.37&\h&\h$\leq19.5$ &\h\nd   &\h\nd  &\h\nd   &\h&\h 17.23&\h 17.0–-17.2
&\h 1($\geq0.89$)    &\h&\h 0.07   &\h N \\
PKS 0736+01          &\h WF2/F675W &\h 1800&\h 16.20&\h 16.93&\h 2.77&\h 4.00
&\h 22.54&\h&\h$\leq20.5$ &\h\nd   &\h\nd  &\h\nd   &\h&\h 16.93&\h 16.7–-17.0
&\h 1($\geq0.96$) &\h&\h 0.04      &\h N \\
PKS 1020$−-$103       &\h WF2/F675W &\h 1800&\h 16.82&\h 17.18&\h 1.68&\h 4.00
&\h 21.69&\h&\h$\leq22.0$ &\h\nd   &\h\nd  &\h\nd   &\h&\h 17.18&\h 17.1–-17.2
&\h 1($\geq0.99$) &\h&\h 0.05      &\h N \\
PKS 1217+02          &\h WF2/F675W &\h 1800&\h 16.31&\h 17.28&\h 2.21&\h 4.00
&\h 22.39&\h&\h$\leq20.5$ &\h\nd   &\h\nd  &\h\nd   &\h&\h 17.28&\h 17.3
&\h 1($\geq0.95$) &\h&\h 0.03      &\h N \\
PKS 2135$−-$14        &\h WF2/F675W &\h 1800&\h 16.27&\h 17.14&\h 2.97&\h 4.00
&\h 22.90&\h&\h$\leq21.0$ &\h\nd   &\h\nd  &\h\nd   &\h&\h 17.14&\h 16.9–-17.0
&\h 1($\geq0.97$) &\h&\h 0.04      &\h N \\
%PKS 2247+14          &\h WF2/F675W &\h 1800&\h 16.76&\h 17.16&\h 2.69&\h 4.00
%&\h 22.70&\h&\h$\leq20.0$ &\h -–   &\h -–  &\h -–   &\h&\h 17.16&\h 17.0–-17.2
%&\h 1($\geq0.93$) &\h&\h 0.01      &\h N \\
PKS 2349$−-$01        &\h WF2/F675W &\h 1800&\h 16.02&\h 16.41&\h 3.04&\h 4.00
&\h 22.22&\h&\h 17.12&\h 3.30      &\h 0.88&\h 22.34&\h&\h 15.96&\h 16.0  
&\h 0.65          &\h&\h 0.69      &\h N \\
PKS 2355$−-$082         &\h WF2/F675W &\h 1800&\h 17.33&\h 17.05&\h 2.13&\h 4.00
&\h 22.09&\h&\h$\leq20.5$ &\h\nd   &\h\nd  &\h\nd   &\h&\h 17.05&\h 16.9–-17.1
&\h 1($\geq0.96$) &\h&\h 0.05      &\h N \\
\tablenotetext{a}{
We list $R_e$, $n$, and $\mu_e$ only for unambiguous disks; otherwise, we
attribute the component to a tidal features, for which only their apparent 
magnitude is given.
}
\enddata
\tablecomments{
Col. (1): Object name.
Col. (2): $HST$ detector and filter.
Col. (3): Exposure time.
Col. (4): Apparent nuclear magnitude at the observed filter.
Col. (5): Apparent bulge magnitude at the observed filter.
Col. (6): Effective radius of bulge.
Col. (7): \ser\ index for bulge.
Col. (8): Surface brightness of bulge at the effective radius
(mag arcsec$^{-2}$).
Col. (9): Apparent magnitude of disk or tidal feature.
Col. (10): Effective radius of disk.
Col. (11): \ser\ index for disk.
Col. (12): Surface brightness of disk at the effective radius
(mag arcsec$^{-2}$).
Col. (13): Apparent host magnitude from combining the luminosity of the bulge 
(Col. 5) and of the disk or tidal features (Col. 9).
Col. (14): Apparent host magnitude from aperture photometry after
subtracting the PSF, determined either by the best-fit PSF or by scaling up
to the maximum value of image.
Col. (15): Bulge-to-total luminosity ratio of host galaxy; upper limit, if
measurable, is shown in parentheses for elliptical galaxies (see text for
details).
Col. (16): Amplitude of the first Fourier mode.
Col. (17): Quality of image: N = normal image; S = saturated image; P= poor
image (pixels near object are useless due to bleeding columns).
}
\end{deluxetable}
%\end{document}



==> tab3.tex <==
%\documentclass[12pt,preprint]{aastex}
%\begin{document}
\pagestyle{empty}
\tiny
\begin{deluxetable}{lcrcc}
\tablecolumns{5}
\tablenum{3}
\tabletypesize{\scriptsize}
\tablewidth{0pc}
\tablecaption{Derived Properties}
\tablehead{
\colhead{ Name} &
\colhead{ $A_V$} &
\colhead{ $M_{R,{\rm nuc}}$} &
\colhead{ $M_{R,{\rm bul}}$} &
\colhead{ $M_{R,{\rm host}}$} \\
\colhead{ } &
\colhead{ (mag)} &
\colhead{ (mag)} &
\colhead{ (mag)} &
\colhead{ (mag)} \\
\colhead{ (1)} &
\colhead{ (2)} &
\colhead{ (3)} &
\colhead{ (4)} &
\colhead{  (5) }
}
\startdata
3C 59&0.211& $-22.71$ & $-22.66_{-  0.3}^{+  0.3}$ &$-22.66_{-  0.3}^{+  0.3}$\nl
E1821+643&0.141& $-27.15$ & $-24.63_{-  0.6}^{+  0.3}$ &$-24.63_{-  0.3}^{+  0.3}$\nl
Fairall 9&0.089& $-18.98$ & $-21.16_{-  0.8}^{+  0.5}$ &$-21.56_{-  0.4}^{+  0.4}$\nl
$[$HB89$]$ 0316$-$346&0.056& $-24.50$ & $-22.86_{-  0.6}^{+  0.6}$ &$-23.14_{-  0.5}^{+  0.5}$\nl
$[$HB89$]$ 2201+315 &0.410& $-25.87$ & $-23.80_{-  0.5}^{+  0.5}$ &$-23.80_{-  0.5}^{+  0.5}$\nl
$[$HB89$]$ 2201+315 &0.410& $-25.91$ & $-24.57_{-  0.5}^{+  0.5}$ &$-24.57_{-  0.5}^{+  0.5}$\nl
HE 0306$-$3301&0.046& $-24.56$ & $-21.71_{-  0.4}^{+  0.4}$ &$-22.65_{-  0.3}^{+  0.3}$\nl
HE 0354$-$5500&0.053& $-24.49$ & $-23.26_{-  0.4}^{+  0.4}$ &$-23.30_{-  0.3}^{+  0.3}$\nl
HE 1434$-$1600&0.417& $-23.38$ & $-22.09_{-  0.3}^{+  0.3}$ &$-22.09_{-  0.3}^{+  0.3}$\nl
MC 1635+119&0.171& $-21.27$ & $-22.47_{-  0.3}^{+  0.3}$ &$-22.47_{-  0.3}^{+  0.3}$\nl
MRK 1048 &0.110& $-21.37$ & $-21.94_{-  0.4}^{+  0.4}$ &$-22.49_{-  0.3}^{+  0.3}$\nl
MS 0244.8+1928&0.368& $-23.26$ & $-22.21_{-  0.3}^{+  0.3}$ &$-22.21_{-  0.3}^{+  0.3}$\nl
MS 0754.6+3928&0.220& $-24.22$ & $-21.92_{-  0.3}^{+  0.3}$ &$-21.92_{-  0.3}^{+  0.3}$\nl
MS 1059.0+7302&0.173& $-21.12$ & $-20.65_{-  0.7}^{+  0.4}$ &$-22.10_{-  0.3}^{+  0.3}$\nl
MS 1545.3+0305&0.377& $-20.48$ & $-21.61_{-  0.7}^{+  0.4}$ &$-22.40_{-  0.4}^{+  0.4}$\nl
OX 169 &0.367& $-24.50$ & $-22.93_{-  0.4}^{+  0.4}$ &$-23.10_{-  0.3}^{+  0.3}$\nl
PG 0052+251&0.157& $-24.12$ & $-22.47_{-  0.4}^{+  0.4}$ &$-22.89_{-  0.3}^{+  0.3}$\nl
PG 0804+761&0.115& $-24.68$ & $-21.66_{-  0.4}^{+  0.4}$ &$-21.78_{-  0.3}^{+  0.3}$\nl
PG 0923+201&0.141& $-24.44$ & $-22.76_{-  0.3}^{+  0.3}$ &$-22.76_{-  0.3}^{+  0.3}$\nl
PG 0953+414&0.042& $-25.41$ & $-22.53_{-  0.3}^{+  0.3}$ &$-22.53_{-  0.3}^{+  0.3}$\nl
PG 1004+130&0.127& $-25.61$ & $-23.84_{-  0.3}^{+  0.3}$ &$-23.84_{-  0.3}^{+  0.3}$\nl
PG 1012+008&0.116& $-23.71$ & $-22.83_{-  0.3}^{+  0.3}$ &$-22.83_{-  0.3}^{+  0.3}$\nl
PG 1116+215&0.075& $-24.78$ & $-23.20_{-  0.3}^{+  0.3}$ &$-23.20_{-  0.3}^{+  0.3}$\nl
PG 1202+281&0.070& $-23.64$ & $-22.40_{-  0.5}^{+  0.5}$ &$-22.40_{-  0.5}^{+  0.5}$\nl
PG 1211+143&0.115& $-23.76$ & $-21.00_{-  0.4}^{+  0.4}$ &$-21.36_{-  0.3}^{+  0.3}$\nl
PG 1226+023 &0.068& $-26.92$ & $-23.85_{-  0.3}^{+  0.3}$ &$-23.85_{-  0.3}^{+  0.3}$\nl
PG 1302$-$102 &0.141& $-26.10$ & $-23.85_{-  0.5}^{+  0.5}$ &$-23.85_{-  0.5}^{+  0.5}$\nl
PG 1302$-$102 &0.141& $-26.00$ & $-23.63_{-  0.5}^{+  0.5}$ &$-23.63_{-  0.5}^{+  0.5}$\nl
PG 1307+085&0.112& $-24.05$ & $-22.14_{-  0.5}^{+  0.5}$ &$-22.14_{-  0.5}^{+  0.5}$\nl
PG 1309+355&0.040& $-24.63$ & $-23.59_{-  0.8}^{+  0.5}$ &$-23.59_{-  0.5}^{+  0.5}$\nl
PG 1351+640&0.068& $-23.43$ & $-22.11_{-  0.4}^{+  0.4}$ &$-22.19_{-  0.3}^{+  0.3}$\nl
PG 1411+442&0.028& $-23.52$ & $-21.24_{-  0.4}^{+  0.4}$ &$-22.11_{-  0.3}^{+  0.3}$\nl
PG 1416$-$129 &0.311& $-22.82$ & $-21.57_{-  0.5}^{+  0.5}$ &$-21.57_{-  0.5}^{+  0.5}$\nl
PG 1426+015 &0.105& $-23.61$ & $-21.51_{-  0.4}^{+  0.4}$ &$-22.75_{-  0.3}^{+  0.3}$\nl
PG 1444+407&0.046& $-25.23$ & $-22.77_{-  0.7}^{+  0.4}$ &$-23.10_{-  0.3}^{+  0.3}$\nl
PG 1613+658&0.088& $-24.33$ & $-23.21_{-  0.4}^{+  0.4}$ &$-23.73_{-  0.3}^{+  0.3}$\nl
PG 1617+175 &0.138& $-23.22$ & $-21.08_{-  0.4}^{+  0.4}$ &$-21.24_{-  0.3}^{+  0.3}$\nl
PG 1700+518&0.116& $-25.97$ & $-24.38_{-  0.4}^{+  0.4}$ &$-24.44_{-  0.3}^{+  0.3}$\nl
PG 2130+099&0.147& $-23.44$ & $-20.68_{-  0.9}^{+  0.6}$ &$-21.61_{-  0.5}^{+  0.5}$\nl
PHL 909&0.151& $-24.34$ & $-23.08_{-  0.3}^{+  0.3}$ &$-23.08_{-  0.3}^{+  0.3}$\nl
PHL 1093 &0.096& $-23.53$ & $-23.62_{-  0.3}^{+  0.3}$ &$-23.62_{-  0.3}^{+  0.3}$\nl
PKS 0736+01&0.422& $-24.12$ & $-23.05_{-  0.3}^{+  0.3}$ &$-23.05_{-  0.3}^{+  0.3}$\nl
PKS 1020$-$103&0.153& $-23.38$ & $-22.89_{-  0.3}^{+  0.3}$ &$-22.89_{-  0.3}^{+  0.3}$\nl
PKS 1217+02&0.070& $-24.29$ & $-23.34_{-  0.3}^{+  0.3}$ &$-23.34_{-  0.3}^{+  0.3}$\nl
PKS 2135$-$14&0.169& $-23.98$ & $-23.05_{-  0.3}^{+  0.3}$ &$-23.05_{-  0.3}^{+  0.3}$\nl
PKS 2349$-$01&0.091& $-23.81$ & $-23.32_{-  0.4}^{+  0.4}$ &$-23.73_{-  0.3}^{+  0.3}$\nl
PKS 2355$-$082&0.133& $-23.02$ & $-23.21_{-  0.3}^{+  0.3}$ &$-23.21_{-  0.3}^{+  0.3}$\nl
\enddata
\tablecomments{
Col. (1): Object name.
Col. (2): Galactic extinction in the $V$ band.
Col. (3): $R$-band absolute magnitude of the nucleus
after correcting for Galactic extinction.
Col. (4): $R$-band absolute magnitude of the bulge and its error
(see text for details).
Col. (5): $R$-band absolute magnitude of the entire host.
}
\end{deluxetable}
%\end{document}


==> tab4.tex <==
%\documentclass[12pt,preprint]{aastex}
%\begin{document}
\pagestyle{empty}
\begin{deluxetable}{ccrc}
\tablecolumns{4}
\tablewidth{0pc}
\tablenum{4}
\tablecaption{$\log M_{\rm BH}/M_\odot = \alpha-0.50 M_{R,{\rm bul}}$}
\tablehead{
\colhead{ Sample} &
%\colhead{ Uncertainties} &
\colhead{ $\alpha$} &
\colhead{ $\Delta \alpha$\tablenotemark{a}} &
\colhead{ Scatter} 
}
\startdata
All &  $-2.87\pm  0.04$& $-0.27$& 0.41\nl
\\
High $L_{\rm bol}/L_{\rm Edd}$ ($\geq 0.1$) &$ -3.08\pm  0.05$& $-0.48$& 0.31\nl
Low $L_{\rm bol}/L_{\rm Edd}$ ($< 0.1$)     & $-2.53\pm  0.06$& $ 0.07$& 0.30\nl
\\
Elliptical ($B/T = 1$)& $-3.04\pm  0.05$& $-0.44$& 0.27\nl
Bulge-dominated ($B/T \geq 0.5$) &$ -2.74\pm  0.07$& $-0.14$& 0.43\nl
Disk-dominated ($B/T < 0.5$) & $-2.26\pm  0.11$& $0.34$& 0.37\nl
\\
No Interaction ($a_1 < 0.3$) & $-2.78\pm  0.04$& $-0.18$& 0.37\nl
Interaction ($a_1 \geq 0.3$) & $-3.33\pm  0.10$& $-0.73$& 0.32\nl
\\
Radio-loud  ($R \geq 10$) & $-3.05\pm  0.07$& $-0.45$& 0.22\nl
Radio-quiet ($R <    10$) & $-2.78\pm  0.05$& $-0.18$& 0.45\nl
\\
$z \leq$ 0.15 & $-2.42\pm  0.04$& $ 0.18$& 0.44\nl
$z >$ 0.15 & $-3.10\pm  0.04$& $-0.50$& 0.28\nl
\enddata
\tablenotetext{a}{
$\Delta \alpha$ compared to the relation of normal galaxies ($\alpha=-2.60$).
}
\end{deluxetable}
%\end{document}

